Edge-exchangeable graphs and sparsity (NIPS 2016)

Many popular network models rely on the assumption of (vertex) exchangeability, in which the distribution of the graph is invariant to relabelings of the vertices. However, the Aldous-Hoover theorem guarantees that these graphs are dense or empty with probability one, whereas many real-world graphs are sparse. We present an alternative notion of exchangeability for random graphs, which we call edge exchangeability, in which the distribution of a graph sequence is invariant to the order of the edges. We demonstrate that edge-exchangeable models, unlike models that are traditionally vertex exchangeable, can exhibit sparsity. To do so, we outline a general framework for graph generative models; by contrast to the pioneering work of Caron and Fox (2015), models within our framework are stationary across steps of the graph sequence. In particular, our model grows the graph by instantiating more latent atoms of a single random measure as the dataset size increases, rather than adding new atoms to the measure.

==> power_laws.tex <==
\label{sec-powerlaw}
We now characterize several types of desirable power laws for graphs.


\TBD{move definitions of graph quantities from the next section here,
    and then briefly discuss Type I, II, and III power laws for edges and
    triangles, make the notation/formatting consistent}



\textbf{Type I power law}:
We first consider power laws in
the asymptotic number of edges as a function of the
asymptotic number of (effective) vertices, and
the asymptotic number of triangle as a function of the
asymptotic number of (effective) vertices.
\begin{align*}
    \text{\textbf{Type Ia:}~~}
\mathcal{E}_N \simas c\,\mathcal{V}_N^a, \, N \rightarrow \infty,
\qquad
    \text{\textbf{Type Ib:}~~}
\mathcal{T}_N \simas c\,\mathcal{V}_N^a, \, N \rightarrow \infty,
\end{align*}
for constants $c > 0, a \in (1,2)$.


\textbf{Type II power law}:
We might also consider power laws in the counts of vertices and triangles.
\begin{align*}
    \text{\textbf{Type IIa:}~~}
\mathcal{D}_{N, r} \simas c\, \mathcal{V}_N^a, \,     N \rightarrow \infty,
\qquad
    \text{\textbf{Type IIb:}~~}
    \mathcal{T}_{N, r} \simas c \, \mathcal{V}_N^a, \, N \rightarrow \infty
\end{align*}

%\textbf{Type IIb power law}: Similarly, we might have a power law in the number
%of vertices with a certain number of triangles
%\begin{align*}
%    \mathcal{T}_{N, r} \simas c \, \mathcal{V}_N^a, \, N \rightarrow \infty
%\end{align*}
Note that $c$ and $a$ need not be the same constants across these power laws.
%
These two types of power laws have behavior similar to Heaps' law
\cite{heaps1978information}
and Zipf's law \cite{zipf1949human} and have been studied extensively in a variety of
real-world data.
Some examples of graphs with this type of power law include the number of hyperlinks
in relation to the number of users (and other variables)
in an internet graph \cite{DBLP:journals/im/Mitzenmacher03} and web caching strategies for
the number of requests for webpages \cite{adamic2002zipf}.



A fundamentally different type of power law
%reminiscent of the kind defined by \citet{MR2934958} for feature modeling
is given by the \emph{distribution} of a quantity on a vertex,
rather than the asymptotic values of counts; the next type of power law gives a
power law in the degree and triangle distribution.

\textbf{Type IIIa power law}:
Power laws
for the degree and triangle distributions at a vertex $i$ is given by:
\begin{align*}
    \text{\textbf{Type IIIa:}~~}
    \Pr(D_{N,i} > M) \sim c M^{-a},
    \qquad
    \text{\textbf{Type IIIb:}~~}
    \Pr(T_{N,i} > M) \sim c M^{-a}.
\end{align*}
%\textbf{Type IIIb power law}: Similarly, we could consider the number of triangles at a vertex $i$:
%\begin{align*}
%    \Pr(T_{N,i} > M) \sim c M^{-a}.
%\end{align*}
%
These types of power laws have been widely studied in
a number of real-world graphs, such as
degrees of proteins in a protein-interaction network of yeast, degrees
of metabolites in the metabolic network of E.\ coli; see
\citet{DBLP:journals/im/Mitzenmacher03, newman2005power,
DBLP:journals/siamrev/ClausetSN09} for more details.
Triangle distribution power laws have been observed in a number of real world
social networks, such as LinkedIn and Twitter, and YahooWeb
\citep{DBLP:conf/pakdd/KangMF11}.



